Improving the generalization of deep learning models in the segmentation of mammography images

Mammography stands as the main screening method for detecting breast cancer early, enhancing treatment success rates. The segmentation of landmark structures in mammography images can aid the medical assessment in the evaluation of cancer risk and the image acquisition adequacy. We introduce a series of data-centric strategies aimed at enriching the training data for deep learning-based segmentation of landmark structures. Our approach involves augmenting the training samples through annotation-guided image intensity manipulation and style transfer to achieve better generalization than standard training procedures. These augmentations are applied in a balanced manner to ensure the model learns to process a diverse range of images generated by different vendor equipments while retaining its efficacy on the original data. We present extensive numerical and visual results that demonstrate the superior generalization capabilities of our methods when compared to the standard training. For this evaluation, we consider a large dataset that includes mammography images generated by different vendor equipments. Further, we present complementary results that show both the strengths and limitations of our methods across various scenarios. The accuracy and robustness demonstrated in the experiments suggest that our method is well-suited for integration into clinical practice.

==> related_work.tex <==
\section{Related work}
\label{sec:related_work}

The estimation of the pectoral muscle is essential for aiding in the assessment of potential abnormalities and the image acquisition correctness. Some deep learning-based methods were proposed to segment the pectoral muscle contour in the MLO view, which is enough for supporting image adequacy assessment \cite{rampun2019breast,soleimani2020segmentation}. For the full pectoral muscle shape segmentation, some approaches considered U-Net architectures \cite{ali2020enhancing,rubio2021multicriteria}, generative adversarial networks \cite{guo2020automatic}, attention mechanisms \cite{yu2022pemnet}, and domain-oriented augmentation operations to achieve better generalization \cite{verboom2024deep}. 

The nipple constitutes another important landmark structure, facilitating the registration of multiple views or modalities by enabling efficient region matching and anatomical measurements. Most of the proposed methods for nipple estimation are hand-crafted, involving the analysis of breast boundary \cite{yin1994computerized, mendez1996automatic, chandrasekhar1997simple, mustra2009nipple}, texture \cite{casti2013automatic}, and convergence of fibroglandular tissue \cite{zhou2004computerized, kinoshita2008radon}. Some data-driven methods were proposed to estimate the nipple position, considering random forest classifiers \cite{jiang2019radiomic} and deep neural networks \cite{lin2019nipple}.

The fibroglandular tissue represents a critical area of concern warranting specific attention during medical assessments. Depending on the patient's unique anatomy, this tissue can exhibit varying characteristics, ranging from dense formations to more dispersed patterns, with higher density correlating to increased risk. Numerous methodologies have been proposed in the existing literature for segmenting dense fibroglandular tissue regions \cite{he2015review}, encompassing both handcrafted \cite{matsubara2001automated,el2010expectation,highnam2010robust,torres2019morphological} and data-driven methods \cite{keller2012estimation,keller2015preliminary,saffari2020fully,larroza2022breast,hu2022breast}.

Several methodologies aim to integrate the segmentation of various landmark structures within a unified framework. Tiryaki et al. conduct experiments employing multiple U-Net-based models to segment the pectoral muscle, dense fibroglandular tissue regions, and fatty tissues \cite{tiryaki2022deep}. In a similar way, considering these structures and incorporating the nipple, Dubrovina et al. introduce a novel deep learning-based framework for comprehensive segmentation tasks \cite{dubrovina2018computational}. By leveraging multiple deep learning models, Bou demonstrates segmentation results encompassing more intricate structures, including vessels, calcifications, and skin, among others \cite{bou2019deep}. 

In a recent development, Sierra-Franco et al. \cite{sierra2024towards} introduced a large dataset alongside deep learning experiments for the segmentation of mammography images, encompassing both MLO and CC views. The study highlights four primary structures of interest in both views: nipple, pectoral muscle, fibroglandular tissue, and fatty tissue. We propose a data-centric approach for the improvement of the generalization of the solution introduced in this work on the processing of mammography images generated by different vendor equipments.

